Compilation Quotient (CQ): A Metric for the Compilation Hardness of Programming Languages

Today's programmers can choose from an exceptional range of programming languages, each with its own traits, purpose, and complexity. A key aspect of a language's complexity is how hard it is to compile programs in the language. While most programmers have an intuition about compilation hardness for different programming languages, no metric exists to quantify it. We introduce the compilation quotient (CQ), a metric to quantify the compilation hardness of compiled programming languages. The key idea is to measure the compilation success rates of programs sampled from context-free grammars. To this end, we fairly sample over 12 million programs in total. CQ ranges between 0 and 100, where 0 indicates that no programs compile, and 100 means that all programs compile. Our findings on 12 popular compiled programming languages show high variation in CQ. C has a CQ of 48.11, C++ has 0.60, Java has 0.27 and Haskell has 0.13. Strikingly, Rust's CQ is nearly 0, and for C, even a large fraction of very sizable programs compile. We believe CQ can help understand the differences of compiled programming languages better and help language designers.

==> graphics/bound-estimation.tex <==
\begin{tikzpicture}[scale=0.7]
    \begin{axis}[
      xlabel={Index (log)},
      ylabel={Program size},
      xmin=0, xmax=13.703768887187252,
      ymin=0, ymax=100,
      grid=both,
      clip=false,
      extra x ticks={12.004798882851654},
      extra x tick labels={$i'_{64}$},
      extra y ticks={64},
      xticklabels={},
      yticklabels={},
      xtick={0},
      ytick={0},
      %x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
      %y label style={at={(axis description cs:-0.17,0.5)},anchor=north},
    ]

    \path[->, very thick] (2,8) edge node[sloped, anchor=center, above] {Below target -- increase estimate} (10.5,23);
    \path[->, very thick, blue] (11.5,83) edge node[anchor=center, left, blue, align=right] {Above target \\ decrease estimate} (11.5,62);
    \addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.0,16)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.3010299956639812,19)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.47712125471966244,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.6020599913279624,20)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.6989700043360189,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.7781512503836436,18)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.8450980400142568,20)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.9030899869919435,21)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.9542425094393249,21)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.0,21)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.041392685158225,22)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.3222192947339193,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.4913616938342726,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.6127838567197355,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.7075701760979363,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.7853298350107671,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.8512583487190752,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.9084850188786497,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.9590413923210936,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.0043213737826426,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.0453229787866576,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.3242824552976926,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.4927603890268375,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.6138418218760693,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.708420900134713,22)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.786041210242554,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.851869600729766,25)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.909020854211156,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.9595183769729982,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.004751155591001,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.0457140589408676,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.3244882333076564,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4929000111087034,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.61394747678035,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.708505880955237,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7861122837198264,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8519306786402674,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.9090744014009045,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.9595660466379274,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.004794110388712,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.045753147594141,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.324508805747058,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.492913970848403,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.613958040857214,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.708514378122784,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.786119390427871,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.851936785958904,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.909079755756776,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.959570813316652,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.004798405634823,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.045757056265976,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.324510862937401,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.492915366797694,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.613959097250767,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.708515227830395,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.786120101092279,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.851937396686044,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.909080291188732,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.959571289981647,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.004798835157097,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.0457574471312245,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.324511068655899,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.492915506392377,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.613959202889982,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.708515312801064,53)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.786120172158656,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.851937457758711,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.909080344731891,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.959571337648118,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.004798878109302,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.04575748621773,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.324511089227744,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.4929155203518425,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.613959213453901,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.7085153212981306,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.786120179265293,55)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.851937463865977,51)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.9090803500862075,53)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.9595713424147645,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.004798882404522,55)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.04575749012638,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.324511091284927,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.49291552174779,54)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.613959214510293,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.708515322147838,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.786120179975956,59)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.851937464476704,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.909080350621638,50)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.95957134289143,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.004798882834043,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.045757490517246,51)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.324511091490647,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.492915521887383,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.613959214615932,54)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.708515322232808,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.786120180047023,52)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.851937464537777,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.909080350675183,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(9.959571342939096,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.004798882876996,57)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.045757490556332,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.324511091511217,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.492915521901343,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.613959214626496,57)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.708515322241306,55)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.78612018005413,55)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.851937464543884,60)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.909080350680536,60)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(10.959571342943862,56)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.00479888288129,53)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.045757490560241,59)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.324511091513276,59)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.49291552190274,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.613959214627553,55)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.708515322242155,57)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.78612018005484,57)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.851937464544495,53)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.909080350681071,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(11.959571342944338,57)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(12.00479888288172,70)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.00479888288129,70)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882880863,69)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882880433,67)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882880003,79)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882879573,69)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882879143,73)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882878715,68)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882878285,70)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882877855,69)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882877425,73)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.00479888287313,71)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882868835,70)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.00479888286454,69)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882860245,73)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.00479888285595,70)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882851654,79)};
\addplot[mark=asterisk, mark size=3, mark options={blue}, only marks] coordinates {(12.004798882847359,62)};
\end{axis}
\end{tikzpicture}


==> graphics/sampling-one-bucket.tex <==
\begin{tikzpicture}[scale=0.7]
    \definecolor{fig3-green}{HTML}{008000}
    \begin{axis}[
      xlabel={Index (log)},
      ylabel={Program size},
      xmin=0, xmax=4.973132473729186,
      ymin=0, ymax=80,
      grid=both,
      clip=false,
      % xmode=log,
      xticklabels={},
      yticklabels={},
      xtick={0},
      ytick={0},
      x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
      y label style={at={(axis description cs:-0.17,0.5)},anchor=north},
    ]
    \draw[densely dashed, black] (0,48) node[left] {48} -- (4.973132473729186, 48);
    \draw[densely dashed, black] (0,32) node[left] {32} -- (4.973132473729186, 32);
    \draw[densely dashed, black] (1.4913616938342726,0) node[below] {$i_{32}'$} -- (1.4913616938342726, 80);
    \draw[densely dashed, black] (3.973174052682972,0) node[below] {$i_{48}'$} -- (3.973174052682972, 80);
    \addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.0,16)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(1.6434526764861874,29)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(1.9395192526186185,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.113943352306837,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.2380461031287955,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.3344537511509307,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.413299764081252,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.4800069429571505,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.537819095073274,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.5888317255942073,23)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.6344772701607315,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.6757783416740852,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.7134905430939424,23)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.7481880270062002,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.780317312140151,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.8102325179950842,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.8382192219076257,29)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(2.864511081058392,37)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(2.88930170250631,37)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(2.912753303671323,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.935003151453655,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.9561684304753633,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.9763499790032735,27)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(2.9956351945975497,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.0273496077747564,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.0610753236297916,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.0923696996291206,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.1215598441875008,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.1489109931093564,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.1746411926604483,32)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.198931869932209,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.2219355998280053,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.243781916093795,29)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.2645817292380777,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.2844307338445193,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.303412070596742,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.3215984304653436,29)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.339053735709139,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.355834495884936,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.371990911464915,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.387567779417189,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4026052419199146,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4171394097273255,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.431202884556517,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4448251995097476,31)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.458033192496506,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4708513245261177,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4892551683692603,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.512817758564873,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.535167485114944,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.556423121371285,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.5766868052009957,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.596047007545439,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.614580866997486,27)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.632356046239073,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.6494322232416168,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.6658623002031554,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.681693392004564,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.696967640744023,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7117228918272347,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7259932589247224,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.739809599021359,27)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.753199914199416,33)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.7661896933101597,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7788022040132385,24)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.7910587435918255,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8029788553352617,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.814580516010319,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8258802989361795,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.836893516376434,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8500945943867007,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8706964579892498,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.890365121448124,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.909181475977853,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.9272163305912646,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.944532020991981,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.9611837098124356,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.977220446635385,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.9926860391621277,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.007619774517403,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.022057020601165,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.036029730656543,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.049566869164652,27)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.062694773342393,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.075437461585613,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.08781689793553,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.099853219884381,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.111564935454498,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.122969094393747,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.134081437462512,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.1449165270928505,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.155487862141282,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.165807979003786,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.175888540992899,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.195152133593287,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.213809844641501,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.2316989107643925,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.248880166024286,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.265407496531089,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.281328859801704,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.296687123772402,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.3115207624480485,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.325864436615346,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.339749481680876,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.35320431990742,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.366254810686386,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.378924549697582,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.39123512565331,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.403206341644807,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.414856406790594,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.42620210284358,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.437258929583457,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.448041232155679,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.458562312981994,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.468834530432752,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.478869386096813,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.488677602194578,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.50505496600964,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.523343191941299,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.540892316015469,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.557759765131784,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.57399652277935,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.58964805833566,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.604755094644832,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.619354246514376,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.63347855533382,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.647157939457867,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.6604195757954745,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.67328822484155,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.685786508921555,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.6979351515051535,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.709753183947856,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.721258124839885,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.732466136205422,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.743392160047862,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.754050038135969,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.76445261744024,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.774611843234153,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.7845388415525,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.7942439924342,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.808082624331254,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.826288656277071,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.8437620828337336,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.860559589976318,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.876731528813316,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.892322825710941,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.9073737346227695,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.92192046335703,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.935995698309741,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.949629046798472,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.962847412052184,35)};
\end{axis}
\end{tikzpicture}


==> graphics/sampling-overlap.tex <==
\begin{tikzpicture}[scale=0.7]
    \definecolor{fig3-green}{HTML}{008000}
    \begin{axis}[
      xlabel={Index (log)},
      ylabel={Program size},
      xmin=0, xmax=8.826794319098209,
      ymin=0, ymax=80,
      grid=both,
      clip=false,
      xticklabels={},
      yticklabels={},
      xtick={0},
      ytick={0},
      x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
      y label style={at={(axis description cs:-0.17,0.5)},anchor=north},
    ]
    \draw [thick,decoration={brace,raise=3pt},decorate] (0.3010299956639812,80) -- node[above=7pt] {bucket \#1} (5.177250723842313,80);
    \draw [thick,decoration={brace,mirror,raise=3pt},decorate] (3.973174052682972,0) -- node[below=7pt] {bucket \#2} (7.826794324922358,0);
    \draw [thick,decoration={brace,mirror, raise=3pt},decorate] (8.826794319098209,32) -- node[right=7pt] {to bucket \#1} (8.826794319098209,48);
    \draw [thick,decoration={brace,mirror, raise=3pt},decorate] (8.826794319098209,48) -- node[right=7pt] {to bucket \#2} (8.826794319098209,64);


    \draw[densely dashed, black] (0,48) node[left] {48} -- (8.826794319098209, 48);
    \draw[densely dashed, gray] (0,32) node[left] {32} -- (8.826794319098209, 32);
    \draw[densely dashed, gray] (0,64) node[left] {64} -- (8.826794319098209, 64);

    \draw[densely dashed, gray] (5.177250723842313,0) -- (5.177250723842313, 80);
    \draw[densely dashed, gray]  (0.3010299956639812,0) -- (0.3010299956639812, 80);
    \draw[densely dashed, gray] (3.973174052682972,0) -- (3.973174052682972, 80);
    \draw[densely dashed, gray]  (7.826794324922358,0) -- (7.826794324922358, 80);
    \addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.0,16)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.110589710299249,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.4099331233312946,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.5854607295085006,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.7101173651118162,20)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.8068580295188172,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.885926339801431,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.952792443044092,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.020775488193558,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.1156105116742996,25)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.1934029030624176,32)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.2593549273080344,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.3165993020938607,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.367169488534681,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.412460547429961,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4534712337229356,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.504198918539445,25)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.568788212315347,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.6250036010148636,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.674769314015426,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7194141597025934,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.759894374025499,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.796921075330169,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8310374856400253,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8794972872494284,31)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.934548947666147,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.983400738180538,31)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.027308827035546,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.067182485523405,31)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.103701119589514,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.13738576433397,30)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.168644776887817,32)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.2184567264004755,38)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.269162565431745,36)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.314562378177839,47)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.35566219858541,38)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.393206554563365,37)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.427761918589799,46)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.459769315966737,39)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.4895788329204365,42)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.542090611555182,33)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.5903624871522615,36)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.633801623517603,36)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.67328822484155,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.709481967073232,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.742890021953482,45)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.773910720232087,37)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.806349587140467,40)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.858639443236375,41)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.9053046610816065,40)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.947438623602977,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(4.985843950580106,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.021127252569096,38)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.053758177841813,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.084107773657156,46)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.120971852128356,48)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.171741076116891,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.217191684154853,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.258333122218849,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.295912199440644,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.330496971331685,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.362529596161941,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.392360992391475,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.433585839649224,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.483092104464963,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.527528081031246,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.567836528446049,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.604719485547809,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.63871383395623,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.670239357167908,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.69963049802918,38)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.745119312295456,54)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.793506115061695,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.837038278149696,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.8766017211886785,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.912860005954602,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.94632303826771,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.977391128489816,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.00638431017859,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.05602355903354,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.10337982055273,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.146076227460703,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.184948241478221,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.220625009314397,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.253592158016637,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.284232379541691,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.314580269066514,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.366521759655511,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.412909394381415,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.454816972835917,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.493034145647045,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.52815859343125,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.560653614820384,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.590885618549694,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.625936994662191,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.6767266147513125,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.722193564929922,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.7633483905724985,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.800938635635752,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.835532865434638,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.867573603029891,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.897412034797226,50)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.937003706046477,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.986696912761666,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.03128340983744,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.0717156553857965,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.108702224232563,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.142784563160466,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.174385740771535,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.203842624225199,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.24781917490132,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.296464951898182,42)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.340206576081499,50)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.379942927714972,63)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.416346368758032,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.44993299016043,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.48110757654714,46)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.510193478164299,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.558407015105629,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.606049895607938,45)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.648979107660398,50)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.6880439679855685,53)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.723883098027579,52)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.756988823539125,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.787748706461174,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.816473310392158,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.8687831612765065,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.915464299148081,52)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.957611237350261,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.996027343340174,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.031319741956855,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.063958446838297,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.094314771955021,56)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.127806650405168,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.178959532022885,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.224717309919614,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.266110230170833,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.303898986970964,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.338661259000725,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.37084608446112,50)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.400809430982317,56)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.438899625354827,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.48894583633808,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.533816244139212,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.57448178416409,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.611663459378372,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.645911383763135,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.67765485476723,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.707235331180346,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.749763931028951,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.798750474060524,49)};
\end{axis}
\end{tikzpicture}


==> graphics/sampling-two-buckets.tex <==
\begin{tikzpicture}[scale=0.7]
    \definecolor{fig3-green}{HTML}{008000}
    \begin{axis}[
      xlabel={Index (log)},
      ylabel={Program size},
      xmin=0, xmax=8.826794319098209,
      ymin=0, ymax=80,
      grid=both,
      clip=false,
      xticklabels={},
      yticklabels={},
      xtick={0},
      ytick={0},
      x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
      y label style={at={(axis description cs:-0.17,0.5)},anchor=north},
    ]
    \draw [thick,decoration={brace,raise=3pt},decorate] (1.4913616938342726,80) -- node[above=7pt] {bucket \#1} (3.973174052682972,80);
    \draw [thick,decoration={brace,raise=3pt},decorate] (3.973174052682972,80) -- node[above=7pt] {bucket \#2} (7.826794324922358,80);


    \draw[densely dashed, black] (0,48) node[left] {48} -- (8.826794319098209, 48);
    \draw[densely dashed, gray] (0,32) node[left] {32} -- (8.826794319098209, 32);
    \draw[densely dashed, gray] (0,64) node[left] {64} -- (8.826794319098209, 64);

    \draw[densely dashed, black] (3.973174052682972,0) node[below] {$i_{48}'$} -- (3.973174052682972, 80);
    \draw[densely dashed, gray] (1.4913616938342726,0) node[below] {$i_{32}'$} -- (1.4913616938342726, 80);
    \draw[densely dashed, gray] (7.826794324922358,0) node[below] {$i_{64}'$} -- (7.826794324922358, 80);
    \addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(0.0,16)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.110589710299249,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.4099331233312946,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.5854607295085006,24)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.7101173651118162,20)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.8068580295188172,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.885926339801431,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(2.952792443044092,26)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.020775488193558,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.1156105116742996,25)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.1934029030624176,32)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.2593549273080344,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.3165993020938607,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.367169488534681,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.412460547429961,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.4534712337229356,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.504198918539445,25)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.568788212315347,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.6250036010148636,28)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.674769314015426,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.7194141597025934,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.759894374025499,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.796921075330169,29)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8310374856400253,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.8794972872494284,31)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(3.934548947666147,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(3.983400738180538,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.027308827035546,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.067182485523405,31)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.103701119589514,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.13738576433397,30)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.168644776887817,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.2184567264004755,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.269162565431745,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.314562378177839,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.35566219858541,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.393206554563365,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.427761918589799,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.459769315966737,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.4895788329204365,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.542090611555182,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.5903624871522615,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.633801623517603,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.67328822484155,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.709481967073232,28)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.742890021953482,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.773910720232087,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.806349587140467,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.858639443236375,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.9053046610816065,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.947438623602977,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(4.985843950580106,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.021127252569096,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.053758177841813,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.084107773657156,46)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.120971852128356,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.171741076116891,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.217191684154853,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.258333122218849,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.295912199440644,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.330496971331685,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.362529596161941,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.392360992391475,32)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.433585839649224,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.483092104464963,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.527528081031246,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.567836528446049,34)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.604719485547809,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.63871383395623,33)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.670239357167908,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.69963049802918,38)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(5.745119312295456,54)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.793506115061695,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.837038278149696,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.8766017211886785,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.912860005954602,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.94632303826771,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(5.977391128489816,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.00638431017859,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.05602355903354,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.10337982055273,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.146076227460703,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.184948241478221,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.220625009314397,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.253592158016637,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.284232379541691,38)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.314580269066514,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.366521759655511,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.412909394381415,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.454816972835917,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.493034145647045,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.52815859343125,39)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.560653614820384,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.590885618549694,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.625936994662191,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.6767266147513125,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.722193564929922,36)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.7633483905724985,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.800938635635752,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.835532865434638,35)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.867573603029891,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(6.897412034797226,50)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.937003706046477,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(6.986696912761666,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.03128340983744,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.0717156553857965,40)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.108702224232563,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.142784563160466,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.174385740771535,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.203842624225199,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.24781917490132,35)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.296464951898182,42)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.340206576081499,50)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.379942927714972,63)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.416346368758032,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.44993299016043,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.48110757654714,46)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.510193478164299,49)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.558407015105629,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.606049895607938,45)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.648979107660398,50)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.6880439679855685,53)};
\addplot[mark=*, mark size=3, mark options={fig3-green}, only marks] coordinates {(7.723883098027579,52)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.756988823539125,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.787748706461174,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.816473310392158,37)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.8687831612765065,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.915464299148081,52)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.957611237350261,46)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(7.996027343340174,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.031319741956855,45)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.063958446838297,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.094314771955021,56)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.127806650405168,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.178959532022885,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.224717309919614,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.266110230170833,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.303898986970964,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.338661259000725,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.37084608446112,50)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.400809430982317,56)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.438899625354827,48)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.48894583633808,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.533816244139212,43)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.57448178416409,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.611663459378372,44)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.645911383763135,47)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.67765485476723,41)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.707235331180346,42)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.749763931028951,49)};
\addplot[mark=x, mark size=3, mark options={black}, only marks] coordinates {(8.798750474060524,49)};
\end{axis}
\end{tikzpicture}


==> res/includes.tex <==



==> res/railroad_diagrams/grammar2railroad <==
#! /usr/local/bin/python3.9

"""
Convert antlr4 grammar into railroad diagram (pdf format).

Prequisites:
    pip install beautifulsoup4
    inkscape
"""

import os
import sys
from bs4 import BeautifulSoup


if len(sys.argv) != 2:
    print("Usage: grammar2railroad <antlr_grammar>")
    exit(1)

rrd_bin="java -jar rrd-antlr4/target/rrd-antlr4-0.1.2.jar "
grammar_file = sys.argv[1]
cmd = rrd_bin + grammar_file
os.system(cmd)

grammar_name = os.path.basename(grammar_file).strip(".g4")
path_prefix = "output/" + grammar_name + "/"
svg_input = open(path_prefix + "/index.html").read()

soup = BeautifulSoup(svg_input, features="html.parser")

# change style
new_style = \
"""
    svg.railroad-diagram {
    }
    svg.railroad-diagram path {
        stroke-width:3;
        stroke:black;
        fill:white;
    }
    svg.railroad-diagram text {
        font:bold 18px monospace;
        text-anchor:middle;
    }
    svg.railroad-diagram text.label{
        text-anchor:start;
    }
    svg.railroad-diagram text.comment{
        font:italic 12px monospace;
    }
    svg.railroad-diagram rect{
        stroke-width:2;
        stroke:black;
        fill:white;
    }
"""
# style_tags = [tag for tag in soup.find_all() if tag.name == "style"]

# for tag in style_tags:
    # tag.string = new_style

svg_tags = [str(tag) for tag in soup.find_all() if tag.name == "svg"]
td_tags = [tag for tag in soup.find_all() if tag.name == "td"]
names = []

for td in td_tags:
    try:
        names.append(td["id"])
    except:
        pass
for idx, tag in enumerate(svg_tags):
    fn = path_prefix + names[idx]+".svg"
    with open(fn, "w") as f:
        f.write(tag)
    cmd = "inkscape " + fn + " -o "+fn.replace("svg", "pdf") #+ " > /dev/null 2&>1"
    os.system(cmd)
    # cmd = "rm -rf " + fn
    # os.system(cmd)
    print(names[idx].split("_")[-1] + " & \\includegraphics[align=t,scale=0.45]{"+"res/railroad_diagrams/"+fn.replace("svg", "pdf") +"}\\\\")

